Conformal Point and the Calibrated Conic

This gives some information about the conformal point and the calibrating conic, and their relationship one to the other. These concepts are useful for visualizing image geometry, and lead to intuitive ways to compute geometry, such as angles and directions in an image.

==> theorenv.tex <==
%
% Derived from article.sty and eccv92.sty
%

\catcode`\@=11

%
%
% New theorem environments
%
%
\newif\if@envcountreset\@envcountresetfalse
\def\ds@envcountreset{\@envcountresettrue}
\def\ts{\thinspace}
%
% new environments and theorems
% borrowed form the LTMP-style of Springer-Verlag
% designed by Dr. Christoph Ender
%
% define the new theorem like environments
% define a new style of environments where it is possible to define
% the font % used as the theorem name and the fontfamily for the text.
%
% \newstytheorem{name}{thefont}{txtfont}{Text}[Counter]
% \newstytheorem{name}{thefont}{txtfont}[oldname]{Text}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
%
\def\newstytheorem#1#2#3{%
\@ifnextchar[{\che@othm{#1}{#2}{#3}}{\che@nthm{#1}{#2}{#3}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@nthm#1#2#3#4{%
\@ifnextchar[{\che@xnthm{#1}{#2}{#3}{#4}}{\che@ynthm{#1}{#2}{#3}{#4}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
% #5 - add theorem counter to reset list of another counter
%
\def\che@xnthm#1#2#3#4[#5]{\expandafter
\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\if@envcountreset\@addtoreset{#1}{#5}\fi
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#4}{#2}{#3}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#2}{#3}{#4}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% change oldthm if oldname in specification is '*'
% then don't use a counter
% #1 - countername
% #2 - theorem font
% #3 - text font
% #4 - counter used
% #5 - string containing theorem name to print
%
\def\che@othm#1#2#3[#4]#5{\expandafter\@ifdefinable
\csname#1\endcsname%
{\@@othm@{#1}{#2}{#3}{#4}{#5}\global\@namedef{end#1}{\@endtheorem}}}
%
\def\@@othm@#1#2#3#4#5{\if *#4{\global\@namedef{the#1}{\relax}
\global\@namedef{#1}{\@bthm@{}{#5}{#2}{#3}}}\else
{\global\@namedef{the#1}{\@nameuse{the#4}}% define the counter
\global\@namedef{#1}{\che@thm{#4}{#5}{#2}{#3}}}\fi}
%
% new defs for theorem environment che 17-MAR-1989
% it improves the option possible
%
% #1 - countername  = theorem name
% #2 - string containing theorem name to print
% #3 - theorem font
% #4 - text font
\def\che@thm#1#2#3#4{\@ifnextchar({\@athm{#1}{#2}{#3}{#4}}{%
\@ifnextchar *{\@bthm{#1}{#2}{#3}{#4}}%
{\@@thm{#1}{#2}{#3}{#4}}}}
%
% \begin{thm}(A.1)[test]      results in:
% \end{thm}                               thm A.1 (test) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - is the new label
% #6 - optional string
%
\def\@athm#1#2#3#4(#5){\@ifnextchar[{%
\@aythm{#1}{#2}{#3}{#4}{#5}}{\@axthm{#1}{#2}{#3}{#4}{#5}}}
\def\@axthm#1#2#3#4#5{\@@locthmlab{#1}{#5}%
\@begintheorem{#2}{#5}{#3}{#4}\ignorespaces}
\def\@aythm#1#2#3#4#5[#6]{\@@locthmlab{#1}{#5}%
\fuh@opargbegintheorem{#2}{#5}{#6}{#3}{#4}\ignorespaces}
%
% \begin{thm}*[xytest]        results in:
% \end{thm}                               thm (xytest) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - optional string
%
\def\@bthm@#1#2#3#4{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bthm#1#2#3#4*{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bxthm#1#2#3#4{\if !#1!\relax\else\@@locthmlab{#1}{}\fi
\@@begintheorem{#2}{#3}{#4}\ignorespaces}
\def\@bythm#1#2#3#4[#5]{%
\@@opargbegintheorem{#2}{#3}{#4}{#5}\ignorespaces}
%
% define local label
%   if no number or a user specified label occured
%
\def\@@locthmlab#1#2{\expandafter\def\csname the#1\endcsname{#2}
\let\@chetempa\protect\def\protect{\noexpand\protect\noexpand}%
\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}%
\let\protect\@chetempa}
%
% #1 - counter = theorem name
% #2 - string with name
% #3 - font for theorem name and label
% #4 - font for text
\def\@@thm#1#2#3#4{\refstepcounter
    {#1}\@ifnextchar[{\che@ythm{#1}{#2}{#3}{#4}}{%
    \che@xthm{#1}{#2}{#3}{#4}}}
%
\def\che@xthm#1#2#3#4{\che@begintheorem{#2}{\csname
the#1\endcsname}{#3}{#4}\ignorespaces}
\def\che@ythm#1#2#3#4[#5]{\che@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}
%
% #1 - name of theorem
% #2 - label string
% #3 - font for name and lable
% #4 - text fomt
%
\def\che@begintheorem#1#2#3#4{#4\trivlist\item[#3 #1\ts #2.]}
%
% #1 - name of theorem
% #2 - label string
% #3 - additonal text
% #4 - font for name and lable
% #5 - text fomt
%
\def\che@opargbegintheorem#1#2#3#4#5{#5 \trivlist
\item[#4 #1\ts #2\ #3.]}
%
\def\fuh@opargbegintheorem#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3).}]}
%
\def\@@begintheorem#1#2#3{#3\trivlist\item[#2 #1.]}
\def\@@opargbegintheorem#1#2#3#4{#3\trivlist\item[#2 #1 #4.]}
 
\newstytheorem{theorem}{\bf}{\it}{Theorem}[section]
\newstytheorem{conjecture}{\bf}{\it}{Conjecture}[section]
\newstytheorem{example}{\bf}{\rm}[theorem]{Example}
\newstytheorem{proposition}{\bf}{\it}[theorem]{Proposition}
\newstytheorem{corollary}{\bf}{\it}[theorem]{Corollary}
\newstytheorem{lemma}{\bf}{\it}[theorem]{Lemma}
\newstytheorem{proof}{\it}{\rm}[*]{Proof}
\newstytheorem{definition}{\bf}{\rm}[theorem]{Definition}
\newstytheorem{remark}{\it}{\rm}[*]{Remark}
\newstytheorem{exercise}{\it}{\rm}[theorem]{Exercise}
\newstytheorem{problem}{\it}{\rm}[theorem]{Problem}
\newstytheorem{solution}{\it}{\rm}[theorem]{Solution}
\newstytheorem{note}{\it}{\rm}[theorem]{Note}
\newstytheorem{question}{\it}{\rm}[theorem]{Question}
\newstytheorem{condition}{\it}{\rm}[theorem]{Condition}
\newstytheorem{algorithm}{\bf}{\rm}[theorem]{Algorithm}
\newstytheorem{numbered}{\bf}{\it}[theorem]{}
\renewcommand{\thenumbered}{(\thesection.\arabic{numbered})}
%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
\newenvironment{unnumbered}{\begin{itemize}\item\em}{\end{itemize}}
\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
 
% qed sign
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\catcode`\@=12

%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
%\renewcommand{\thenumbered}{(\thechapter.\arabic{numbered})}

%
% symbol for end of example
%
% \def\endexample{\hspace*{1em \@plus 1000fil}\nolinebreak\examplebox\endlist}
\def\endtheorem{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endexample{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endproposition{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endcorollary{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endlemma{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\enddefinition{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endremark{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endexcse{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endproblem{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endsolution{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endnote{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endquestion{\hspace*{\fill}\nolinebreak\examplebox\endlist}
\def\endcondition{\hspace*{\fill}\nolinebreak\examplebox\endlist}

\def\endproof{\hspace*{\fill}\nolinebreak\squareforqed\endlist}
\def\endresult{\hspace*{\fill}\nolinebreak\examplebox\endlist}
% \def\examplebox{\begin{picture}(6.5,6.5)%
% \put(0,0){\framebox(6.5,6.5){}}\end{picture}}
% \def\examplebox{{$\Diamond$}}
\def\examplebox{{$\triangle$}}
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}



